Fast Benchmarking of Accuracy vs. Training Time with Cyclic Learning Rates

Benchmarking the tradeoff between neural network accuracy and training time is computationally expensive. Here we show how a multiplicative cyclic learning rate schedule can be used to construct a tradeoff curve in a single training run. We generate cyclic tradeoff curves for combinations of training methods such as Blurpool, Channels Last, Label Smoothing and MixUp, and highlight how these cyclic tradeoff curves can be used to evaluate the effects of algorithmic choices on network training efficiency.

==> miscellaneous.tex <==
	
% In many instances, the CLR tradeoff curve underestimated the standard tradeoff curve by a margin of $\sim$0.5\% validation accuracy.  There are many possible variations to our approach that might improve this gap. Some ideas for future directions include allowing the entire cyclic learning rate schedule to decay over the course of learning by decreasing the maximum learning rate after each reset. This is one of many schedule variations explored by the literature \citep{schmidt2021descending}. Another idea is to apply Stochastic Weight Averaging (SWA, Izmailov et al., 2018) at the end of each cycle. This would entail, at the end of each trough, cycling the learning rate (even more!) at low amplitude and at high frequency, and averaging the weights. Such an approach might boost the validation accuracy and lead to Pareto optimality in some instances. Another idea would involve repeating linear warm up instead of a hard reset, although it is unclear if this would improve accuracy. We found that sawtooth/triangular cyclic learning rate schedules did not get close to the Pareto frontier for ResNet-50 on ImageNet (data not shown).

% We could also experiment with other multiplier values. The behavior of the PyTorch \texttt{CosineAnnealingWarmRestarts} scheduler makes it difficult to control the spacing of points sampled along the tradeoff curve, in part due to the constraint of epoch-wise (and not step-wise) scheduling. We hope to circumvent this problem in future versions of Composer. Future approaches could also apply a cyclic learning rate to other hyperparameters such as weight decay, batch size, and gradient clipping, in line with \cite{smith2022general}.

% Our cyclic learning rate approach to constructing tradeoff curves worked nicely for training methods such as Blurpool and Label Smoothing. However, in the current implementation of MosaicML Composer (or PyTorch), it won’t work for methods that have their own independent schedules such as Layer Freezing \citep{brock2017freezeout}, Stochastic Weight Averaging (SWA) \citep{izmailov2018averaging}, and Progressive Resizing (Fast.ai). It can work in principle, however, if the schedules for methods such as Progressive Resizing cycle with the learning rate schedule. We hope to implement this in future versions of the library.

% The use of Pareto frontiers in ML research is surprisingly limited, and is mostly restricted to the subfield of multi-objective optimization (MOO) for multitask learning (some recent examples include \cite{lin2020controllable,navon2020learning}). We have found that thinking about Pareto optimality is useful for framing more fundamental questions in neural network training.




% Constructing a tradeoff curve allows us to then make claims such as:

% \begin{itemize}
%     \item For a desired accuracy A, the network should be trained for a particular amount of time T
%     \item Given a time budget T, accuracy A can be achieved
% \end{itemize}

% We consider one configuration to be better than another if the tradeoff curve it produces is further upward and to the left (e.g., the \textit{crimson curve} in the Figure \ref{fig:fig-teaser}B). 


%Cyclic learning rate schedules were popularized by Fast.ai \citep{howard2020fastai}, but are not widely used in the research community. This is likely due to the fact that, with current best practices on benchmarks like ImageNet, cyclic learning rate schedules do not necessarily lead to improved or even commensurate accuracy when compared to cosine decay schedules (data not shown). And while some of the early motivation for cyclic learning rates was to be able to interrupt training at any time and still return good performance (a.k.a. an “anytime” algorithm), anytime performance is not necessarily of interest for heavily studied benchmarks with known, standard hyperparameters.



%However, characterizing different points on a tradeoff curve can be computationally expensive; a naive implementation requires training a new model from scratch for every single point on the curve. 

%This often makes it difficult to compare results across papers and make meaningful progress within particular subfields \cite{blalock2020state}.



%\subsection{Predicting Training Performance with Accuracy-Training Time Tradeoff Curves}

%It is particularly useful to frame neural network training as a tradeoff between accuracy and time. 



% Constructing a Pareto frontier curve allows us to then make predictions such as:

% \begin{itemize}
% \item For a desired accuracy A, the network should be trained for N epochs
% \item Given a time budget of N epochs, accuracy A can be achieved
% \end{itemize}

% For example, in Figure 1B, we can see that if we want to reach a validation accuracy of $77\%$ on ImageNet with ResNet-50, we need to train for at least 7 hours (SSR Baseline, blue line). We can also see that, given a budget of 2.25 hours, we should expect an accuracy of $74.5\%$ (SSR Baseline, blue line).

% Pareto frontier curves also allow us to make quantitative statements about different hyperparameter choices and training algorithms, for example:

% \begin{itemize}
% \item Method L, (e.g. Channels Last) shifts the Pareto frontier along the time axis, leading to speedup for the same accuracy
% \item Method M (e.g. image augmentation method MixUp) increases the Pareto frontier along the quality axis, leading to improvements in accuracy for the same amount of training time
% \end{itemize}

% For example, in Figure 1B, a training recipe consisting of Blurpool (Zhang 2019), Channels Last, Label Smoothing (Szegedy et al. 2015, Müller et al. 2015), and MixUp (Zhang et al. 2017) both shifts the Pareto frontier to the left, and increases the accuracy for the same number of training epochs. This sort of comparison is much more informative than a table of numbers.

% If we define each point on the Pareto frontier curve as a single training run, as above, then densely sampling N points on the curve entails N separate training runs of different durations. The question of efficiency then becomes: given a fixed recipe for training (e.g. architecture, objective function, regularization methods), how can we efficiently estimate the Pareto frontier?



%We use this approach extensively in the MosaicML Explorer benchmarking across cloud instances, hardware choices, and speedup methods. However, the added expense of doing so was especially painful given that we performed thousands of training runs to collect this data.

% A single point on a “Pareto frontier” curve represents a single training run with a particular training recipe on a specific hardware instance (e.g. training ResNet-50 on ImageNet for 90 epochs with linear warmup and cosine decay, batch size 2048, gradient accumulation of 4, on eight RTX 3080 GPUs, etc.). In order to construct a Pareto-optimal tradeoff curve, we can vary a single parameter - training duration - and scale the learning rate schedule appropriately while keeping everything else the same (Figure 1A). Constructing this curve therefore entails training multiple copies of a single network with different training durations and learning rate schedules. Armed with these data points, we can construct a single curve which maps training time to accuracy. This can be done across architectures (e.g. ResNet-50, ResNet-101) and training algorithms such as Label Smoothing (Szegedy et al. 2015, Müller et al. 2015) and MixUp (Zhang et al. 2017), for a single task such as ImageNet. Importantly, a tradeoff curve constructed by training a single model with a decaying learning rate is not Pareto-optimal for many vision tasks and therefore not particularly useful (as can be seen from the validation accuracy curves in Figure 1A). 




%(C) Training with Blurpool, Channels Last, Label Smoothing and MixUp (BP+CL+LS+MX, \textit{crimson}) leads to a Pareto improvement for all training times. This means that for a given number of epochs, this combination of training methods will lead to an increase in accuracy and a decrease in training time (i.e. a shift up and to the left).
